TiFi: Taxonomy Induction for Fictional Domains [Extended version]

Taxonomies are important building blocks of structured knowledge bases, and their construction from text sources and Wikipedia has received much attention. In this paper we focus on the construction of taxonomies for fictional domains, using noisy category systems from fan wikis or text extraction as input. Such fictional domains are archetypes of entity universes that are poorly covered by Wikipedia, such as also enterprise-specific knowledge bases or highly specialized verticals. Our fiction-targeted approach, called TiFi, consists of three phases: (i) category cleaning, by identifying candidate categories that truly represent classes in the domain of interest, (ii) edge cleaning, by selecting subcategory relationships that correspond to class subsumption, and (iii) top-level construction, by mapping classes onto a subset of high-level WordNet categories. A comprehensive evaluation shows that TiFi is able to construct taxonomies for a diverse range of fictional domains such as Lord of the Rings, The Simpsons or Greek Mythology with very high precision and that it outperforms state-of-the-art baselines for taxonomy induction by a substantial margin.

==> sections/6-discussion.tex <==
\section{Discussion}

\simoncomment{This section is important since the method is our contribution. What do we learn from the experiments? Which features work/do not work, how well does the method generalize, how difficult is (hyper-)parameter tuning, etc.}
\todoC{Can be removed. The feature analysis is already in above sections}

==> tables-end.tex <==

\begin{table}%[!htpb]
\centering
\scalebox{0.95}{
\begin{tabular}{l|c|c|c}
\hline
\textbf{Universe} & \textbf{\#New Types} & \textbf{\#New Edges} & \textbf{Precision} \\ \hline
LoTR     & 43                          & 171                       & 0.84                  \\ \hline
GoT      & 39                          & 179                       & 0.84                  \\ \hline
Starwars      &         373                  &       3387                 &      0.84             \\ \hline
Simpsons      &          115                 &       439                 &      0.92             \\ \hline
World of Warcraft      &     257                      &       2248                 &      0.84             \\ \hline
Greek Mythology      &      22                     &       76                 &        0.84           \\ \hline
\end{tabular}
} % end scalebox
\caption{WordNet Integration Results.}
\label{tab:exp-wordnet-integration}
\end{table}





\begin{table}%[!htpb]
\centering
\begin{tabular}{l|c|c|c}
\hline
\textbf{Universe} & \textbf{\# Types} & \textbf{\# Edges} & \textbf{Precision} \\ \hline
LoTR              &         353          &          648         &     0.88               \\ \hline
Game of Thrones   &         292          &          497         &       0.83             \\ \hline
Star Wars         &         7352          &         12282          &     0.90               \\ \hline
Simpsons      &             1029      &             2171      &        0.88            \\ \hline
World of Warcraft            &      4063             &      7882             &        0.76            \\ \hline
Greek Mythology & 139 & 313 & 0.91 \\ \hline
\end{tabular}
\caption{Taxonomies produced by TiFi.}
\label{tab:fantasy-taxonomy-statistics}
\end{table}



\begin{table}%[!htpb]
\centering
\scalebox{1}{
\begin{tabular}{c|r|r|r|r}
\hline
\textbf{}              & \multicolumn{2}{c|}{\textbf{Text}}                                         & \multicolumn{2}{c}{\textbf{Structured Sources}}                                  \\ \hline
\textbf{Query}         & \multicolumn{1}{c|}{\textbf{Google}} & \multicolumn{1}{c|}{\textbf{Wikia}} & \multicolumn{1}{c|}{\textbf{Wikia-categories}} & \multicolumn{1}{c}{\textbf{TiFi}} \\ \hline
\multicolumn{1}{c|}{$t$} & 2 (52\%)                              & 7 (65\%)                             & 10 (62\%)                                     & 8 (87\%)                            \\ \hline
\multicolumn{1}{c|}{$t_1 \cap t_2$} & 1 (23\%)                              & 2 (11\%)                             & 8 (40\%)                                      & 3 (70\%)                            \\ \hline
\multicolumn{1}{c|}{$t_1 \setminus t_2$} & 1 (20\%)                              & 4 (36\%)                             & 8 (63\%)                                      & 6 (79\%)                            \\ \hline
\textbf{Average}       & 1 (32\%)                              & 4 (37\%)                             & 9 (55\%)                                      & 6 (79\%)                            \\ \hline
\end{tabular}}
\caption{Avg. \#Answers and Precision of Entity Search.} %\simoncomment{Add space between answer count and precision.}
\label{tab:entity-search-results}
\end{table}




\begin{table*}%[!t]
\centering
\scalebox{0.55}{
\begin{tabular}{l|c|c|l|l}
\hline
\textbf{}              & \multicolumn{2}{c|}{\textbf{Text}}                                         & \multicolumn{2}{c}{\textbf{Structured Sources}}                                  \\ \hline
\multicolumn{1}{c|}{\textbf{query}}                                                       & \textbf{Google}                                                                                                      & \textbf{Wikia}                                                                                  & \multicolumn{1}{c|}{\textbf{Wikia-categories}}                                                                                                                                                                                                                                                                                                                                                                                    & \multicolumn{1}{c}{\textbf{TiFi}}                                                                                                                                                                                                                                        \\ \hline
Dragons in LOTR                                                                            & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Glaurung, T\'{u}rin Turambar, \\ Ancalagon, E\"{a}rendil, Smaug\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Dragons, \sout{Summoned Dragon}, \\ Spark-dragons\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\sout{Urgost},Long-worms,Gostir,\sout{Drogoth the Dragon Lord},\sout{Cave-Drake},\\ \sout{War of the Dwarves and Dragons}, \sout{Dragon-spell},Stone Dragons,\\ Fire-drake of Gondolin,Spark-dragons,Were-worms,\sout{Summoned Dragon},\\ Fire-drakes,Glaurung,Ancalagon,Dragons,Cold-drakes,Sea-serpents,\\ \sout{User blog:Alex Lioce/Kaltdrache the Dragon},Smaug,\sout{Dragon (Games Workshop)},\\\sout{Drake},Scatha,\sout{The Fall of Erebor}\end{tabular} & \begin{tabular}[c]{@{}l@{}}Long-worms ,Gostir,\sout{War of the Dwarves and Dragons},\\ \sout{Dragon-spell},Stone Dragons ,Fire-drake of Gondolin ,\\ Spark-dragons,Were-worms,Fire-drakes,Glaurung,Ancalagon,\\ Dragons,Cold-drakes,Sea-serpents,Smaug,Scatha ,\sout{The Fall of Erebor}\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Which Black Numenoreans \\ are servants of Morgoth\end{tabular} & -                                                                                                                    & Black N\'{u}men\'{o}rean                                                                                               & \begin{tabular}[c]{@{}l@{}}Men of Carn D\^{u}m,Corsairs of Umbar,Witch-king of Angmar,\\ \sout{Thrall Master},Mouth of Sauron,Black N\'{u}men\'{o}rean,Fuinur\end{tabular}                                                                                                                                                                                                                                                                & \begin{tabular}[c]{@{}l@{}}Men of Carn D\^{u}m,Corsairs of Umbar,Witch-king of Angmar,\\ Mouth of Sauron,Black N\'{u}men\'{o}rean,Fuinur\end{tabular}                                                                                                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}Which spiders \\ are not agents of Saruman?\end{tabular}        & -                                                                                                                    & -                                                                                                  & \begin{tabular}[c]{@{}l@{}}Shelob ,\sout{Spider Queen and Swarm},\sout{Saenathra},\\\sout{Spiderling},Great Spiders,\sout{Wicked, Wild, and Wrath}\end{tabular}                                            & Shelob,Great Spiders    \\ \hline
\end{tabular}}
\caption{Example queries and results for the entity search evaluation.}%\simoncomment{Unify with Table 9: Remove Wikidata, add Wikia category network.}
\label{tab:entitysearch}
\end{table*}
